Elliptic Units Above Fields With Exactly One Complex Place

In this work we explore the construction of abelian extensions of number fields with exactly one complex place using multivariate analytic functions in the spirit of Hilbert's 12th problem. To this end we study the special values of the multiple elliptic Gamma functions introduced in the early 2000s by Nishizawa following the work of Felder and Varchenko on Ruijsenaars' elliptic Gamma function. We construct geometric variants of these functions enjoying transformation properties under an action of $\mathrm{SL}_{d}(\mathbb{Z})$ for $d \geq 2$. The evaluation of these functions at points of a degree $d$ field $\mathbb{K}$ with exactly one complex place following the scheme of a recent article by Bergeron, Charollois and Garc\'ia (arXiv:2311.04110) seems to produce algebraic numbers. More precisely, we conjecture that such infinite products yield algebraic units in abelian extensions of $\mathbb{K}$ related to conjectural Stark units and we provide numerical evidence to support this conjecture for cubic, quartic and quintic fields.

==> computing/orientations.tex <==
\subsection{Orientations}\label{orientations}

To state the conjecture properly, we must discuss the orientations, that is to say the choice of signs $\mu_{\rho}, \nu_{\rho}$. The cycle we use to evaluate our $G_r$ functions is mimics the cycle used in \cite{Colmez}, \cite{Diazydiaz} in the context of explicit Shitani cones in totally real fields, as well as in \cite{Sczech} in the context of the Eisenstein cocycle for totally real fields. Therefore, we choose orientations to mimic the orientations given in \cite{Colmez}. Remember that we have fixed a set $\eps_1, \dots, \eps_r$ of fundamental units for $\opc{\goth{f}}$. We have also fixed the ordering of the real embeddings so we may consider the sign of the regulator of these units.
$$sg(\eps_1, \dots, \eps_r) = sign(\det(\log(\sigma_{j}(\eps_k))_{1 \leq j,k \leq r}))$$

\begin{general}{Definition}\label{deforientations}
The sign of the unit system $\eps_1, \dots, \eps_r$ is defined by:
$$sg(\eps_1, \dots, \eps_r) = sign(\det(\log(\sigma_{j}(\eps_k))_{1 \leq j,k \leq r}))$$
Then, the signs in Conjecture \ref{conjecture} are defined for all $\rho \in \goth{S}_r$  by
$$\mu_{\rho} = \nu_{\rho} = sg(\eps_1, \dots, \eps_r) \signature(\rho)$$
where $\signature(\rho)$ is the signature of the permutation $\rho$.
\end{general}

%We now introduce a special character to complete our choice of signs. In the setting of Stark's conjecture for ATR fields, if $\kk$ contains a unit $\eps$ such that $\eps \equiv 1 \mod \goth{f}$ and $\norm{\eps} = -1$ then all partial $\zeta$ functions associated to $\goth{f}$ have a zero of order at least $2$ at $0$. Then we may consider only the case where $\kk$ contains no such unit. Consider the set 
%$$\zz_{\goth{f}}^1 = \{n \in \zz, (n, \goth{f}) = 1, \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f} \}$$
%This set contains $1$ and is stable by multiplication. Moreover, if an integer $n$ belongs to this $\zz_{\goth{f}}^1$, then $n+qk$ still belongs to $\zz_{\goth{f}}^1$ for all $k \in \zz$, where $\goth{f} \cap \zz = q\zz$. Take $n \in \zz_{\goth{f}}^1$. Then if $\eps, \eps'$ are two units such that $n\eps \equiv n \eps' \equiv 1 \mod \goth{f}$ then $\norm{\eps}$ and $\norm{\eps'}$ must be the same. We may then define 


%To state the conjecture properly, we must discuss the orientations, that is to say the choice of basis $B_L$, and the choice of signs $\mu_{\rho}, \nu_{\rho}$. We will first discuss the choice of global orientation of the field $\kk$ and then discuss the choice of signs $\mu_{\rho}, \nu_{\rho}$.

%Remember that we have fixed a complex embedding $\sigma_{\cc}$ of $\kk$. Consider any element $x \in \kk$ which doesn't belong to any subfield of $\kk$ such that $\sigma_{\cc}$ sends $x$ to the upper half-plane. Suppose further that $\sigma_1(x) < \sigma_2(x) < \dots < \sigma_r(x)$. Then the Vandermonde matrix
%$$\begin{pmatrix} 1 & 1 & \dots &1& 1 \\ x^{(1)} & x^{(2)} & \dots &x^{(r+1)} & x^{(r+2)}\\ \dots & \dots & \dots & \dots & \dots \\  x^{(1)^{d-1}} & x^{(2)^{d-1}} & \dots &x^{(r+1)^{d-1}} & x^{(r+2)^{d-1}} \end{pmatrix} $$
%has determinant $-ik\sqrt{|D|}$ where $D$ is the discrimant of the field $\kk$ and $k \in \qq_>0$. This justifies our choice of positive bases.

%From now on we fix an order on the real embeddings of $\kk$ and we define a basis $B = (e_1, \dots, e_d)$ of $\kk$ to be positive if $\det((e_i^{(j)})_{1 \leq i, j \leq d})$ lies in the lower half-plane. We will now fix a $\zz$-basis $B_L$ for the $\zz$-module $L$ that is a positive $\qq$-basis of $\kk$.  

%We now discuss the choice of signs $\mu_{\rho}, \nu_{\rho}$. The cycle we use to evaluate our $G_r$ functions is mimics the cycle used in \cite{Colmez}, \cite{Diazydiaz} in the context of effective Shitani cones in totally real fields. Therefore, we keep orientations that resemble the orientations given in \cite{Colmez}. Remember that we have fixed a set $\eps_1, \dots, \eps_r$ of fundamental units for $\opc{\goth{f}}$. We have fixed the ordering of the real embeddings so we may consider the sign of the regulator of these units:
%$$sg(\eps_1, \dots, \eps_r) = sign(\det(\log(\eps_i^{(j)})_{1 \leq i,j \leq r}))$$
%We now introduce a special character to complete our choice of signs. In the setting of Stark's conjecture for ATR fields, if $\kk$ contains a unit $\eps$ such that $\eps \equiv 1 \mod \goth{f}$ and $\norm{\eps} = -1$ then all partial $\zeta$ functions associated to $\goth{f}$ have a zero of order at least $2$ at $0$. Then we may consider only the case where $\kk$ contains no such unit. Consider the set 
%$$\zz_{\goth{f}}^1 = \{n \in \zz, (n, \goth{f}) = 1, \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f} \}$$
%This set contains $1$ and is stable by multiplication. Moreover, if an integer $n$ belongs to this $\zz_{\goth{f}}^1$, then $n+qk$ still belongs to $\zz_{\goth{f}}^1$ for all $k \in \zz$, where $\goth{f} \cap \zz = q\zz$. Take $n \in \zz_{\goth{f}}^1$. Then if $\eps, \eps'$ are two units such that $n\eps \equiv n \eps' \equiv 1 \mod \goth{f}$ then $\norm{\eps}$ and $\norm{\eps'}$ must be the same. We may then define 

%\begin{general}{Definition}
%$$\mathcal{Z}_{\goth{f}}^1 = \begin{cases} \{n \in \left(\zz/q\zz\right)^{\times}, n \leq (q-1)/2, \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f} \} & \mathrm{if~} d \equiv 0 \mod 2 \\ \{n \in \left(\zz/q\zz\right)^{\times}, \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f}\} & \mathrm{if~} d \equiv 1 \mod 2 \end{cases} $$
%$$\mathcal{Z}_{\goth{f}}^1 = \{n \in \left(\zz/q\zz\right)^{\times}, \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f}\}$$
%$$\chi := \begin{cases} \mathcal{Z}_{\goth{f}}^1 & \to \{\pm 1\} \\ n & \to \begin{cases} 1 &\mathrm{~if~}\exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f} \mathrm{~with~} \norm{\eps} = 1 \\ -1 &\mathrm{~if~} \exists\,\eps \in \ok^{\times}, n\eps \equiv 1 \mod \goth{f} \mathrm{~with~} \norm{\eps} = -1 \end{cases} \end{cases}$$
%\end{general}

%\noindent One checks easily that $\mathcal{Z}_{\goth{f}}^1$ is a subgroup of $(\zz/q\zz)^{\times}$, that it contains $-1$ and that $\chi(-1) = (-1)^d$. We use this character and the sign of the regulator to define the orientations in our conjecture.

%\begin{general}{Definition}\label{deforientations}
%The signs in Conjecture \ref{conjecture} are defined for all $\rho \in \goth{S}_r$ and all $n \in \mathcal{Z}_{\goth{f}}^1$ by
%$$\mu_{\rho, n} = \nu_{\rho,n } = \chi(n) sg(\eps_1, \dots, \eps_r) \signature(\rho)$$
%where $\signature(\rho)$ is the signature of the permutation $\rho$.
%\end{general}






























==> computing/target.tex <==
\subsubsection{Target ideals}

%In this section we make the assumptions of \pendingref and we fix a permutation $\rho \in \goth{S}_r$. We wish to understand what happens when a given prime number $p$ divides $\ts$. Let us first start with the cubic case. Under the above assumptions, multiplication by $\eps$ in a suitable basis of $\ok$ can be written as 
%$$\eps = \begin{pmatrix}  0 & u_1 & v_1 \\ 1 & u_2 & v_2 \\ 0 & \pm \tilde{s} & v_3 \end{pmatrix}$$
%This means that $\talpha_0 = m_0 \mp v_3 \teone + \ts \tetwo$ and $\talpha_0\pm v_3\eps-m_0 \in p\ok$. Here we singled out the role of $\talpha_0$ but a similar statement holds for $\talpha_1$, namely $\eps \talpha_1 + v'_3 \eps + m_1 \in p\ok$.
%To generalise this, we will write this condition as 
%$$p\ok \bigcap \{u_j\talpha_j + m_0 + m_1\eps, (m_0, m_1) \in \zz^2\} \neq \emptyset$$
%where $u_0 = 1$ and $u_1 = \eps$. Conversely, it is easy to check that if such a relation is satisfied by $\eps$ then $p$ divides $\tilde{s}$. More generally, for $d \geq 4$ we have the same condition in this specific case :

%\begin{general}{Proposition}
%Under the assumptions \pendingref, the prime divisors of $\ts$ are exactly the primes satisfying 
%$$p\ok \bigcap \{u_j\talpha_j + \sum_{i = 0}^r m_i u_i \in \zz^2\} \neq \emptyset$$
%for some $0 \leq j \leq r$. Furthermore, if this condition is satisfied for $j_0$, it is satisfied for all $j$.
%\end{general}

%\begin{proof}
%Indeed, $\ta u_j \talpha_j = \ttt$ by definition. Now we write $\delta_{kj} = \ta u_k u_j \talpha_j$ and then putting 
%$$ \beta_j = \ttt u_j\alpha_j - \sum_{k = 1}^{r} \delta_{kj} \alpha_k$$
%one gets $\ta u_l(\beta_j) = 0$ for all $1 \leq l \leq r$ and $\ta(\beta_j) = \ttt^2$. This means that $\beta_j - \ttt \talpha_0 \in \zz$. Recall that we may choose the positive basis $[1, u_1, \dots, u_r, v]$ of $L$ in this specific case and that the component of $\talpha_k$ along $v$ is $0$ whenever $k \neq 0$ so that 
%$$u_j \alpha_j = \sum_{i = 0}^{r} m_i u_i + \ttt v$$
%and $u_j \alpha_j - \sum_{i = 0}^{r} m_i u_i \in \ttt \ok$. Conversely, if $p$ satisfies the above condition then there exists a linear combination
%$$u_j \talpha_j + \sum_{i = 0}^r m_i u_i \in p \ok$$
%$$\ta \left(u_j \talpha_j + \sum_{i = 0}^r m_i u_i\right) = \ttt \in p \zz$$
%\end{proof}

While choosing the vector $h = h_{\rho}$, we must be very careful of the value of the overflow $\ttt = \ttt_{\rho}$. Indeed, for most admissible vectors $h$, the constant $\ttt$ depending only on $u_1, \dots, u_r$ will divide $t = t(u_1, \dots, u_r ; h)$ and the computations will require $t^r$ evaluations of ordinary $G_r$ functions, which can become quickly overwhelming. We now introduce the notion of target ideal to understand how to choose $h$ such that $t = 1$. Explicitly, we explain that there is a tradeoff with an increase of the level $l$ as we diminish the value of $t$. In the rest of this section we will make extensive use of the following definitions:

\begin{general}{Definition}\label{ppart}
Let $x \in \kk$ and $I$ be an ideal such that $\norm{I}$ is a power of the prime number $p$. We say that the $p$-part of $x \in \kk$ is the ideal $I$ if for all prime ideal $\goth{P}$ above $p$, $v_{\goth{P}}(x) = v_{\goth{P}}(I)$. 
\end{general}

\begin{general}{Definition}
Let $I$ be a non zero integral ideal in $\ok$ such that $I \cap \zz = n\zz$. Then, for all $\alpha \in \ok$ congruent to an integer modulo $I$ we write $\rmd{\alpha}{I}$ for the unique integer $0 \leq \rmd{\alpha}{I} < |n|$ such that $\alpha-\rmd{\alpha}{I} \in I$.
\end{general}

The number $\rmd{\alpha}{I}$ is naturally called the remainder of $\alpha$ mod $I$. Note that if $I$ is a product of degree one primes above different prime numbers, then all elements $\alpha\in\ok$ are congruent to integers mod $I$.

\begin{general}{Definition}
Let $I$ be a non zero integral ideal in $\ok$. Then, there is a unique primitive ideal $I^{c}$ and a unique integer $n > 0$ such that $II^{c} = n\ok$. We call $I^{c}$ the complementary ideal of $I$.
\end{general}

Before we define the notion of target ideal, we prove a lemma which we will need to control the $p$-adic valuation of the integer $\lambda$ in the construction of section \ref{geomsetup}.

\begin{general}{Lemma}\label{lemmalambda}
Take $h = mh'$ an admissible element in $L$. Suppose that there is a linear combination 
$$\left(u_j + \sum_{i = 0}^{j-1} n_i u_i\right)h' \in p^kL$$
where $j \geq 1$ and the coefficients $n_i$ are integers. Then $p^k$ divides the integer $c_{jj0}$ and therefore $p^k$ divides the integer $\lambda$.
\end{general}

\begin{proof}
Recall that the basis $B_L = (e_0, \dots, e_{r+1})$ defined at the beginning of section \ref{geomsetup} is such that $e_0 = h'$ and for all $1 \leq i \leq r$, $u_ih' = \sum_{k = 0}^i c_{ik0}e_k$ where the $c_{ik0}$ are integers and $c_{ii0} > 0$. This means that 
$$\left(u_j + \sum_{i = 0}^{j-1} n_i u_i\right)h' = c_{jj0}e_j + \left(\sum_{k = 0}^{j-1} c_{jk0} e_k\right) + \sum_{i = 0}^{j-1} \left(\sum_{k = 0}^{i} n_ic_{ik0} e_k\right) \in p^kL$$
so the coordinate of this element on the vector $e_j$ is exactly $c_{jj0}$ and $p^k$ divides $c_{jj0}$. Recalling that $\lambda = \prod_{j = 1}^r c_{jj0}$, we get $p^k$ divides $\lambda$.
\end{proof}




We now define the notion of target ideal to deal with the $p$-adic valuation of the overflow $\ttt$.

\begin{general}{Definition}\label{deftarget}
Let $I$ be a non zero primitive integral ideal of $\ok$ such that $II^c = p^{k_0}\ok$. We say that $I$ is a target ideal associated to the unit system $u_0 = 1, u_1, \dots, u_r$ if the two following conditions are satisfied:
\begin{itemize}
\item there is a linear combination $u_r + \sum_{j= 0}^{r-1}n_j u_j \in I^{c}$ with $n_j \in \zz$
\item for all $0 \leq j \leq r$, $\talpha_j$ is congruent to an integer $n'_j$ modulo $I^c$
\end{itemize}
\end{general}

Note that if the first condition is satisfied or if the second condition is satisfied for some $j$ when $I$ is a degree one prime then necessarily $p | \ttt$. Indeed, in the first case, $\talpha_r - \rmd{\talpha_r}{I} \in I$ so that $(u_r + \sum_{j = 0}^{r-1} n_j u_j)(\talpha_r -\rmd{\talpha_r}{I}) \in p\ok$ and
$$\ttt = \ta u_r\talpha_r = \ta\left(u_r + \sum_{j = 0}^{r-1} n_j u_j\right)(\talpha_r-\rmd{\talpha_r}{I}) \in p\zz$$
In the second case, $u_j -\rmd{u_j}{I} \in I$, so that $(u_j - \rmd{u_j}{I})(\talpha_j - n'_j) \in p\ok$ and $\ta(u_j - \rmd{u_j}{I})(\talpha_j-n'_j) = \ta u_j \talpha_j = \ttt \in p \zz$. The importance of target ideals is expressed by the following lemma.

\begin{general}{Lemma}\label{lemmatarget}
Suppose $(\ast)$. Let $p$ be a prime number such that $v_p(\ttt) > 0$ and suppose that $I$ is a target ideal with $II^c = p^{k_0}\ok$ where $k_0 \geq v_p(\ttt)$ for the unit system $u_0, \dots, u_r$. Suppose further that $\norm{I} = p^{2k_0-v_p(\ttt)}$. Take $h$ an admissible vector with $p$-part exactly $I$. Then $v_p(\lambda) = v_p(l) = k_0$ and $v_p(t) = 0$.
\end{general}

\begin{proof}
The ideal $I$ is a target ideal therefore there are integers $n_0, \dots, n_{r-1}$ such that $(u_r + \sum_{j = 0}^{r-1} n_ju_j)h' \in I^cI = p^{k_0}\ok$. Using lemma \ref{lemmalambda} we obtain that $p^{k_0}$ divides $c_{rr0}$ and so $p^{k_0}$ divides $\lambda$. On the other hand, from lemma $\ref{tmin}$ there is an index $j$ such that $p$ does not divide $\alpha_j + mh'$ for all $m \in \zz$ and from Proposition \ref{propl} there is an integer $m_j$ such that $\epsilon l\alpha_j = \talpha_jh' + m_jh'$ for some  sign $\epsilon = \pm 1$. The ideal $I^c$ is a target ideal, therefore there is an integer $n'_j$ such that $\talpha_j - n'_j \in I^c$. This implies that $\epsilon l\alpha_j - m_jh' - n'_jh' = (\talpha_j -n'_j)h' \in p^{k_0}\ok$. Suppose for now that $p$ does not divide $l$. Then $\exists m \in \zz$ such that $\epsilon lm - m_j - n'_j \in p\zz$. Therefore $\epsilon l(\alpha_j-mh') = (\talpha_j -n'_j)h' + (m_j + n'_j - \epsilon lm)h' \in p\ok$ but this is a contradiction. Therefore $p$ must divide the integer $l$. We then prove by induction that $p^2, \dots, p^{k_0}$ divide $l$. Indeed, if $p^k | l$ with $k < k_0$ then $\epsilon l\alpha_j - (m_j+n'_j)h' \in p^{k_0}\ok$ which means that $m_j + n'_j \in p^{k}\zz$. Suppose that $l \not\in p^{k+1}\zz$. Then there is an integer $m \in \zz$ such that $\epsilon lm - m_j - n'_j \in p^{k+1}\zz$ and then $\epsilon l(\alpha_j -mh') \in p^{k+1}\ok$ which yields again a contradiction. Now, using formula \refp{formulafundam} one finds
$$v_p(\lambda) + v_p(l) + v_p(t) = v_p(\mathcal{N}(h')) - v_p(\mathcal{N}(L)) + v_p(\tlambda) + v_p(\ttt)$$
$$v_p(\lambda) + v_p(l) + v_p(t) = (2k_0-v_p(\ttt)) - 0 + 0 + v_p(\ttt),~~v_p(\lambda) \geq k_0, v_p(l) \geq k_0$$
And this leads to $v_p(\lambda) = k_0$, $v_p(l) = k_0$ and $v_p(t) = 0$. Note once again the most important case where $I$ is a degree one prime and $v_p(\ttt) = 1$. Then we have $v_p(\tlambda) = 1$, $v_p(l) = 1$ and $v_p(t) = 0$.
\end{proof}

This allows us to strengthen the conditions under which we might understand special values of arithmetic $G_r$ functions. We add to the conditions ($\ast$)  the following conditions ($\ast\ast$):
\begin{itemize}
\item for all $\rho \in \goth{S}_r$, for all $p | \ttt_{\rho}$, there exists a target ideal $I_{\rho, p}$  for the unit system $[\eps_{\rho(1)}|\dots| \eps_{\rho(r)}]$ such that $I_{\rho, p}I_{\rho, p}^c = p^{k_0}\ok$ and $\norm{I_{\rho, p}} = p^{2k_0-v_p(\ttt_{\rho})}$
\item for all $\rho \in \goth{S}_r$, there exists an integer $k_{\rho}$ coprime to $q$ such that the class of $k_{\rho}\prod_{p|\ttt} I_{\rho, p}$ in the wide class group of $\kk$ is independent of $\rho$
\end{itemize} 
We discuss briefly what we expect from the conditions ($\ast$) and ($\ast\ast$). In regards to our computations for now, the most restrictive conditions would be the content condition $\tlambda_{\rho} = 1$, as well as the conditions $\norm{\goth{f}} = q = \ell^k$ and $\ttt_{\rho}$ coprime to $q$ as together they rule out many possible ideals $\goth{f}$. The condition $\ts_{\rho} = \ttt_{\rho}$ is expected to be true quite often. Finally, we expect the condition $(\ast\ast)$ to be true generally under the conditions ($\ast$). Note that there may be more than one target ideal for each prime number $p$ dividing the overflow $\ttt_{\rho}$.















==> cubic_case.tex <==
\section{Cubic case}

We start by describing the geometric construction for the cubic case. Let $\kk$ be a cubic complex field and consider a fractional ideal $L$ of $\kk$. Write 
$$\opc{L} = \{\eps \in \units, \eps \equiv 1 \mod L, \eps > 0\}$$
This set is a free $\zz$-module of rank 1 and we write $\eps$ its generator whose real embedding lies in $(0,1)$. Choose $\gamma$ a primitive vector in $L$. Then, there exists a basis of $B_L = [\gamma, e_1, e_2]$ of $L$ such that $\eps\gamma = \mu\gamma+c_1e_1$ and $\eps e_1 = u_0\gamma +u_1e_1+c_2e_2$ with $c_1 >0$ and $c_2 > 0$. We write the multiplication by $\eps$ in this basis as 
$$\eps = \begin{pmatrix} \mu & u_0 & v_0 \\ c_1 & u_1 & v_1 \\ 0 & c_2 & v_2  \end{pmatrix}$$
Now consider $a$ the primitive linear form with same orientation in the line spanned in $\Lambda = \dualsimple{L}$ by $\det(\gamma, \eps\gamma, \cdot)$ and we write $\lambda a = det(\gamma, \eps\gamma, \cdot)$ with $\lambda > 0$. In the above basis, we have $a = [0, 0, 1]$ and $a\eps = [0, c_2, v2]$. We then have $\det(a, a\eps, \cdot) = c_2\gamma = s\gamma$. We define
$$ t = \min\{m \in \zz_{>0}, \exists \alpha_0, \alpha_1 \in L, \abar \alphabar = m I_{2}\}$$
Here we have once again $t = c_2$ and we can choose $\alpha_0 =-v_2e_1+c_2e_2, \alpha_1 = -e_1$. The object we want to consider is then the $\Gamma$ function :
$$\Gamma_{a, a\eps}^{(N)}(\gamma/q, \sigma_{\cc}, \Lambda) = \prod_{F/\zz\gamma}\Gamma^{(N)}\left(\frac{1}{q}, \sigma_{\cc}\left(\frac{\alpha_0}{\gamma}\right), \sigma_{\cc}\left(\frac{\alpha_1}{\gamma}\right)\right) $$
where $q\zz = \zz \cap L$ and $\sigma_{\cc}$ is one of the two conjugated complex embeddings of $\kk$ and $N$ corresponds to a smoothing.

We analyse now $\alphabar$ more closely. We have $\alpha_1 =- e_1 = -(\eps-\mu)\gamma/c_1$ and 
$$\begin{aligned}
\alpha_0 & = \eps e_1 + (v_2 - u_1) e_1 - u_0\gamma \\
\alpha_0 & = \eps (\eps -\mu)\gamma/c_1 + (v_2-u_1)(\eps-\mu)\gamma/c_1 - u_0\gamma \\
\alpha_0 & = \eps^2\gamma/c_1 + (v_2-u_1-\mu)\gamma/c_1 - (\mu(v_2-u_1)/c_1 + u_0)\gamma
\end{aligned}$$
so that the quotients $\alpha_0/\gamma$ and $\alpha_1/\gamma$ depend rather loosely upon $\gamma$. Thus, we are lead to consider the case $\gamma = 1$ and we will try to understand what happens for $\gamma \neq 1$ afterwards. In what follows, we will denote with a $\tilde{}$ everything related to $\gamma = 1$. Consider then $L = \ok$ and $\gamma = 1$. There is a basis $[1, e_1, e_2]$ of $\ok$ such that $\eps = \tilde{\mu} + \tilde{c_1}e_1$. Then the matrix corresponding to the multiplication by $\eps$ is given by
$$\eps = \begin{pmatrix} \tilde{\mu} & \tilde{c_1} u_0 & \tilde{c_1} v_0 \\
\tilde{c_1} & \tilde{c_1} u_1 + \tilde{\mu} & \tilde{c_1} v_1 \\
0 & \tilde{c_1}\tilde{c_2} & \tilde{c_1} v_2 + \tilde{\mu} \end{pmatrix}$$ 
This gives $\tilde{a} = [0, 0, 1], \tilde{a}\eps = [0, \tilde{c_1}\tilde{c_2}, \tilde{c_1} v_2 + \tilde{\mu}]$ and then $\tilde{\lambda} = \tilde{c_1}$, $\tilde{s} = \tilde{t} = \tilde{c_1}\tilde{c_2}$ and $\tilde{\alpha}_0 = (\tilde{c_1}v_2 + \tilde{\mu})e_1 + \tilde{c_1}\tilde{c_2}e_2$, $\tilde{\alpha}_1 = - e_1$. 
On the other hand, $\talpha_0, \talpha_1$ must satisfy the conditions
$$\det(1, \eps, \eps\talpha_0) = 0,~\det(1, \eps, \talpha_1) = 0$$
which means that $\talpha_0 = m_0 + n_0\eps^{-1}$ and $\talpha_1 = m_1 + n_1\eps$. We check easily that $m_1 = \tmu/\tcone$, $n_1 = -1/\tcone$,
$m_0 = -\tcone(v_1\tctwo+u_1v_2)-\tmu(u_1+v_2)-\tmu^2/\tcone$ and $n_0 = 1/\tcone$.
















==> geometric_setup.tex <==
\section{Geometric Setup}
In their article \pendingref, Nicolas Bergeron, Pierre Charollois and Luis Garcia generalise the construction of elliptic units above complex quadratic fields to complex cubic fields using the elliptic $\Gamma$ function from Ruijsenaars. Making use of the work on this function carried out by Felder-Varchenko \pendingref and Felder, \pendingref as well as some generalisation of the elliptic $\Gamma$ function by Nishizawa \pendingref and Narukawa \pendingref, we propose a further generalisation of elliptic units above ATR fields.

\input{geometric_setup/quadratic}
\input{geometric_setup/cubic}
\input{geometric_setup/grfunctions}
\input{geometric_setup/generaldegree}


==> geometric_setup/cubic.tex <==
\subsection{Cubic case}

\input{geometric_setup/cubic/general}
\input{geometric_setup/cubic/lattices}
\input{geometric_setup/cubic/fullconstruction}




==> geometric_setup/cubic/fullconstruction.tex <==
\subsubsection{Full construction}

We now consider the construction carried out in \cite{BCG} to produce conjectural elliptic units above complex cubic fields. We consider a complex cubic field $\kk$ and an integral ideal $\goth{f} \neq \ok$. We write $q\zz = \zz \cap \goth{f}$. The unit group
$$\opc{\goth{f}} = \{\eps \in \units, \eps \equiv 1 \mod L, \eps > 0\}$$
is a free $\zz$-module of rank 1, and we fix $\eps$ its generator whose real embedding belongs to (0,1). We fix an integral ideal $\goth{b}$ prime to $\goth{f}$ and we put $L = \goth{f}\goth{b}^{-1}$. We also fix an integral ideal $\goth{a}$ such that $\goth{a}^{-1}L/L$ is a cyclic group. We call such an ideal a \textit{smoothing} ideal and we write $N$ for the norm of $\goth{a}$. We fix $h \in L$ a vector satisfying $h/q -1 \in L$ and $h/N$ generates the cyclic group $\goth{a}^{-1}L/L$.

We fix a basis $B$ for $L$ and consider the linear form $\det_B(h, \eps h, \cdot)$. We write $\lambda a = \det_B(h, \eps h, \cdot)$ where $\lambda$ is a positive integer and $a \in \Lambda = \dualsimple{L}$ is primitive. Then, fixing a basis $C$ of $\Lambda$ we have $\det_C(a, a\eps, \cdot) = s\gamma$ where $s$ is a positive integer, $\gamma$ is a primitive vector in $L$ and $h$ is a multiple of $\gamma$. We define
$$\Gamma_{\goth{f}, \goth{b}, \goth{a}}(\eps, h, \sigma_{\cc}) = \Gamma_{a, a\eps}(h, \sigma_{\cc}, L)^N/\Gamma_{a, a\eps}(h, \sigma_{\cc}, \goth{a}^{-1}L)$$
This special value of the $\Gamma$ function was related to a special value of the partial $\zeta$ functions in \cite{BCG} as follows. We denote by $[\goth{b} ]$ the class of $\goth{b}$ in $Cl^{+}(\goth{f})$ the narrow ideal class group mod $\goth{f}$. The partial $\zeta$ function associated to this class is
$$\zeta_{\goth{f}}([\goth{b}], s) = \sum_{I \in [\goth{b}]} \norm{I}^{-s}$$ when $\Re(s) > 1$. This function can be extended into a holomorphic function over $\cc$ except possibly at $s = 1$. In the specific case where $\kk$ is complex cubic, this partial $\zeta$ function vanishes at the origin. In \cite{BCG} the authors have proven that

\begin{generalbis}{Theorem}{in \cite{BCG}}
The modulus of $\Gamma_{\goth{f}, \goth{b}, \goth{a}}(\eps, h, \sigma_{\cc})$ is independent of the choice of $h$ and
$$N\zeta'_{\goth{f}}([\goth{b}], 0) - \zeta'_{\goth{f}}([\goth{a}\goth{b}], 0) = \log\left|\Gamma_{\goth{f}, \goth{b}, \goth{a}}(\eps, h, \sigma_{\cc})\right|^2$$
\end{generalbis}

They also conjectured that $\Gamma_{\goth{f}, \goth{b}, \goth{a}}(\eps, h, \sigma_{\cc})$ is a unit in the associated class field $\kk^{+}(\goth{f})$ related to the conjectural Stark unit, and we will present this in section \pendingref.




































==> geometric_setup/cubic/general.tex <==
\subsubsection{The $\Gamma$ function}

The elliptic $\Gamma$ function was first introduced by Ruijsenaars and was studied later at length by Felder and Varchenko who made the connexion with elliptic $\theta$ functions.

\begin{general}{Definition}
For $z \in \cc$ and $\tau, \sigma \in \hh$ put
$$\Gamma(z,\tau,\sigma) = \prod_{m,n \geq 0}\left(\frac{1-\exp(2i\pi((m+1)\tau +(n+1)\sigma-z))}{1-\exp(2i\pi(m\tau+n\sigma+z))} \right)$$
\end{general}

\noindent This function converges absolutely for $z \in \cc, z \not\in \zz +\zz_{\leq 0}\tau + \zz_{\leq 0}\sigma$ and it is holomorphic in this domain. 
The range of parameters can be extended to $\tau, \sigma \in \cc - \rr$ by putting :
$$\Gamma(z, -\tau, \sigma) = \frac{1}{\Gamma(z + \tau, \tau, \sigma)}$$

\begin{generalbis}{Theorem}{[3.1 and 4.1 in \cite{FV}]}
If $\tau, \sigma \in \cc-\rr$ then
\begin{align}
\Gamma(z + 1, \tau, \sigma) = \Gamma(z, \tau + 1, \sigma) & = \Gamma(z, \tau, \sigma+1) = \Gamma(z, \tau, \sigma) \nonumber \\
\Gamma(z + \tau, \tau, \sigma) & = \theta_0(z, \sigma)\Gamma(z, \tau, \sigma) \nonumber \\
\Gamma(z + \tau + \sigma, \tau, \sigma) & = \Gamma(-z, \tau, \sigma)^{-1} \nonumber
\end{align}
Finally, if $\sigma/\tau \not\in \rr$ then
\begin{equation} \label{modgamma}
\Gamma(z, \tau, \sigma)^{-1}\Gamma\left(\frac{z}{\tau}, \frac{-1}{\tau}, \frac{\sigma}{\tau}\right) \Gamma\left(\frac{z-\tau}{\sigma}, -\frac{\tau}{\sigma}, -\frac{1}{\sigma}\right)^{-1} = \exp(i\pi P_1(z,\tau, \sigma))
\end{equation}
where $$P_1(z, \tau, \sigma) = \frac{z^3}{3\tau\sigma} - \frac{\tau + \sigma - 1}{2\tau\sigma}z^2 + \frac{\tau^2 + \sigma^2 + 3\tau\sigma - 3\tau - 3\sigma + 1}{6\tau\sigma}z $$
$$+ \frac{1}{12}(\tau + \sigma - 1)\left(\frac{1}{\tau} + \frac{1}{\sigma} - 1\right)$$ 
\end{generalbis}




















==> geometric_setup/cubic/lattices.tex <==
\subsubsection{Elliptic gamma functions associated to wedges}

In \cite{FDuke} the authors have build elliptic gamma functions associated to wedges in the $\cc^3$ space, and we shall briefly present their construction here.
Consider two primitive vectors $a,b$ in $L = \zz^3$, linearly independent. Fix a basis $B$ of $L$ and write $\det_B(a,b,\cdot) = s\gamma$ for a unique integer $s>0$ and a unique linear form $\gamma \in \Lambda = \dualsimple{L}$. Now write
$$C(a,b) = \{\delta \in \Lambda, \delta(a) > 0, \delta(b) \leq 0\}$$
The elliptic $\Gamma_{a,b}$ function associated to the pair $(a,b)$ is defined as follows.

\begin{general}{Definition}
Let $a,b \in L$ be primitive, independent. We put 
$$\Gamma_{a,b}(w, x) = \frac{\prod_{\delta \in C(a,b)/\zz\gamma}(1-\exp(-2i\pi(\delta(x) - w)/\gamma(x)))}{\prod_{\delta \in C(b,a)/\zz\gamma}(1-\exp(2i\pi(\delta(x) - w)/\gamma(x)))}$$
where $w \in \cc$ and $x \in L_{\cc}$. In the special case $a = b$ we put $\Gamma_{a,a}(w, x) =1$, and we leave the case $\Gamma_{a,-a}$ which is never well-defined.
\end{general}

The study of the convergence properties of this function was carried out in \cite{FDuke} and is better understood with an alternative definition of this function. Consider $\alpha, \beta \in \Lambda$ such that $\alpha(a) > 0, \beta(a) = 0, \alpha(b) = 0, \beta(b) > 0$ and write 
$$ F = \{\delta \in \Lambda, 0 \leq \delta(a) < \alpha(a), 0 \leq \delta(b) < \beta(b)\}$$
Then, we have the following alternative definition.

\begin{generalbis}{Proposition}{\pendingref in \pendingref}
\begin{equation}\label{productformula}\Gamma_{a,b}(w, x) =  \prod_{\delta \in F/\zz\gamma} \Gamma\left(\frac{w+\delta(x)}{\gamma(x)}, \frac{\alpha(x)}{\gamma(x)}, \frac{\beta(x)}{\gamma(x)}\right)
\end{equation}
Furthermore, the right-hand side is independent of the choice for $\alpha, \beta$ and converges for suitables $w$ whenever $\alpha(x)/\gamma(x)$ and $\beta(x)/\gamma(x)$ are not real.
\end{generalbis}
\textbf{Remark : } This proposition can be used to extend the definition of $\Gamma_{a,b}$. Note that we could have taken this to be the definition from the start. This will be done later when considering $G_r$ functions associated to $r+1$ vectors in $\zz^{r+2}$. It will remain to check that this definition is independent of the choice for $\alpha, \beta$, and this can be done by direct computation in reverting the proof of this proposition.

Note that the function $\Gamma_{a,b}$ is here computed as a product of $\#|F/\zz\gamma|$ regular elliptic $\Gamma$ functions. A standard choice gives $\alpha(a) = \beta(b) = s = \#|F/\zz\gamma|$. This choice is given by considering a third vector $c$ such that $\det_B(a,b,c) = s$ and writing the transpose of the comatrix of $(a,b,c)$ as $(\alpha, \beta, s\gamma)^{T}$. 

The properties of the $\Gamma$ function translate into nice properties for the $\Gamma_{a,b}$ functions under the action of $\slnz{3}$. Namely:

\begin{generalbis}{Theorem}{[3.8 in \cite{FDuke}]}
In the domains where every term converges, we have the following inversion relation:
$$\Gamma_{a,b}(w, x)\Gamma_{b,a}(w,x) = 1$$
as well as the following three-term relation
$$\Gamma_{a,b}(w, x)\Gamma_{b,c}(w,x)\Gamma_{c,a}(w,x) = \exp\left(-\frac{i\pi}{3} P_{a,b,c}(w,x)\right)$$
where $P_{a,b,c}$ is a polynomial in $w$ of degree 3. Furthermore, we have the equivariance relations : for all $g \in \slnz{3}$,
$$\Gamma_{ga, gb}(w, gx) = \Gamma_{a, b}(w,x)$$
$$P_{ga, gb, gc}(w,gx) = P_{a,b,c}(w,x)$$
\end{generalbis} 























==> geometric_setup/generaldegree.tex <==
\subsection{Degree $\geq 4$}

\pending write $G_{r, \goth{f}, \goth{b}, \goth{a}}(u_1, \dots, u_r ; \gamma)$

==> geometric_setup/grfunctions.tex <==
\subsection{$G_r$ functions}

\pending write Gr functions then Gr functions in lattices

\input{geometric_setup/grfunctions/general}
\input{geometric_setup/grfunctions/lattices}
\input{geometric_setup/grfunctions/fullconstruction}


































==> geometric_setup/grfunctions/fullconstruction.tex <==
\subsubsection{Gr full construction}

We now consider a generalisation of the construction carried out in section \pendingref. We consider a degree $d \geq 2$ ATR field $\kk$ and an integral ideal $\goth{f} \neq \ok$. We write $q\zz = \zz \cap \goth{f}$. The unit group
$$\opc{\goth{f}} = \{\eps \in \units, \eps \equiv 1 \mod L, \eps > 0\}$$
is a free $\zz$-module of rank $r$, and we fix $(\eps_1, \dots, \eps_r)$ a system of fundamental units of $\opc{goth{f}}$. We fix an integral ideal $\goth{b}$ prime to $\goth{f}$ and we put $L = \goth{f}\goth{b}^{-1}$. We also fix an integral ideal $\goth{a}$ such that $\goth{a}^{-1}L/L$ is a cyclic group. We call such an ideal a \textit{smoothing} ideal and we write $N$ for the norm of $\goth{a}$. We fix $h \in L$ a vector satisfying $h/q -1 \in L$ and $h/N$ generates the cyclic group $\goth{a}^{-1}L/L$.

We fix a basis $B$ for $L$ and we also fix for now $u_1, \dots, u_r \in \opc{\goth{f}}$ such that the linear form $\det_B(h, u_1 h, \dots, u_r h, \cdot)$ is non degenerate. This means that it should be non-zero and that if $\kk$ contains a real subfield, none of the $u_i$ may be real \pendingref. We write as before $\lambda a = \det_B(h, u_1 h, \dots, u_r h, \cdot)$ where $\lambda$ is a positive integer and $a \in \Lambda = \dualsimple{L}$ is primitive. Then, fixing a basis $C$ of $\Lambda$ we have $\det_C(a, au_1, \dots, au_r, \cdot) = s\gamma$ where $s$ is a positive integer, $\gamma$ is a primitive vector in $L$ and $h$ is a multiple of $\gamma$. We define
$$G_{r, \goth{f}, \goth{b}, \goth{a}}(u_1, \dots, u_r ; h, \sigma_{\cc}) = G_{r, (a, au_1, \dots, au_r)}(h, \sigma_{\cc}, L)^N/G_{r, (a, au_1, \dots, au_r)}(h, \sigma_{\cc}, \goth{a}^{-1}L)$$

This generalises the construction of \cite{BCG} and we hope to relate this element to the partial $\zeta$ functions mod $\goth{f}$. Now, in \cite{BCG} they use the Eisenstein cocyle for $\slnz{3}$ to establish the link and it is most likely that the link for $d \geq 4$ will be given by the Eisenstein cocyel for $\slnz{d}$. In view of the work of Sczech in \pendingref we will further compute 

$$I_{\goth{f}, \goth{b}, \goth{a}}(\eps_1, \dots, \eps_r ; h, \sigma_{\cc}) = \prod_{\rho \in \goth{S}_{r}} G_{r, \goth{f}, \goth{b}, \goth{a}}([\eps_{\rho(1)} | \dots | \eps_{\rho(r)}] ; h, \sigma_{\cc})$$
where
$$[\eps_1 | \dots | \eps_r] = \left(\eps_1, \eps_1\eps_2, \dots, \prod_{i=1}^r\eps_i\right)$$



















==> geometric_setup/grfunctions/general.tex <==
\subsubsection{General Gr}

In \cite{Nishizawa} Nishizawa introduced the hierarchy of $G_r$ functions that generalize both the $\theta_0$ and the elliptic $\Gamma$ functions. Later, Narukawa proved the modularity property for $G_r$ by relating it to multiple sine functions. We shall first define these functions then sum up these properties.
To simplify the notations, we will write as in \cite{Nishizawa}, with a clear separation for base and exponential variables :
\begin{align*}
\taubar = (\tau_j)_{0 \leq j \leq r}~&;~\qbar = (q_j)_{0 \leq j \leq r} = (\exp(2i\pi \tau_j))_{0 \leq j \leq r} \\
|\taubar| = \sum_{j = 0}^r \tau_j~&;~|\qbar| = \prod_{j = 0}^r q_j \\
\taubar^{-}(j) = (\tau_n)_{0 \leq n \neq j \leq r}~&;~\qbar^{-}(j) = (q_n)_{0 \leq n \neq j \leq r} \\
\taubar[j] = (\tau_0, \dots, \tau_{j-1}, -\tau_j, \tau_{j+1}, \dots, \tau_r)~&;~\qbar[j] = (q_0, \dots, q_{j-1}, q_j^{-1}, q_{j+1}, \dots, q_r) 
\end{align*}
$$\taubar +_{k} a = (\tau_0, \dots, \tau_{k-1}, \tau_k + a, \tau_{k+1}, \dots, \tau_r)$$
$$f(\taubar) = (f(\tau_j))_{0 \leq j \leq r}$$
$$ \mbar + \bars{1} = (m_j + 1)_{0 \leq j \leq r},~\mbar\taubar = (m_j\tau_j)_{0 \leq j \leq r},~\qbar^{\mbar} = (q_j^{m_j})_{0 \leq j \leq r}$$
$$ \prod_{\mbar \geq 0} = \prod_{m_0 \geq 0} \dots \prod_{m_r \geq 0}$$

\begin{general}{Definition}
Let $r \geq 0$ and $\taubar \in \hh^{r+1}$. For $z \in \cc$, ($z \not\in \zz + \sum_{j=0}^r \zz_{\leq 0}\tau_j$ if $r$ is odd), put $x = \exp(2i\pi z)$ and
$$ G_r(z, \taubar) = \prod_{\mbar \geq 0} \left(1 - \left|\qbar^{\mbar +\onebar}\right|x^{-1}\right)\left(1-\left|\qbar^{\mbar}\right|x\right)^{(-1)^r}$$
\end{general}

\noindent It is clear from this writing that $\theta_0 = G_0$ and $\Gamma = G_1$. Let us summarize the properties satisfied by the $G_r$ functions.

\begin{generalbis}{Theorem}{[3.2 and 3.5 in \cite{Nishizawa}]}
Let $r \geq 1$. Then we have :
\begin{align}
G_r(z+1, \taubar) & = G_r(z, \taubar) = G_r(z, \taubar +_j 1) \nonumber \\
G_r(z + \tau_j, \taubar) & = G_{r-1}(z, \taubarsj{j})G_{r}(z, \taubar) \nonumber \\
G_r(z + |\taubar|, \taubar) & = G_r(-z, \taubar)^{(-1)^r} \nonumber 
\end{align}
\end{generalbis}

\noindent Furthermore, the domain of definition of $G_r$ can be extended with parameters $\tau_j \in \cc-\rr$ by putting 
\begin{equation}\label{inversionGr}
G_r(z, \taubar[j]) = G_r(z + \tau_j, \taubar)^{-1}
\end{equation}
The modular property for the $G_r$ functions was later proved by Narukawa, as we present now. First, let us introduce the multiple Bernoulli polynomials and other useful functions:

\begin{general}{Definition}
Let $\omegabar = (\omega_1, \dots, \omega_r)$ with $\omega_j \neq 0$ for all $1 \leq j \leq r$. We define the multiple Bernoulli polynomials with the following generating function:
$$\frac{t^re^{zt}}{\prod_{j=1}^r (e^{\omega_jt}-1)} = \sum_{n \geq 0} B_{r,n}(z, \omegabar)\frac{t^n}{n!} = \sum_{n \geq 0} \frac{z^nt^n}{n!}\prod_{1 \leq j \leq r} \left(\sum_{n \geq 0} B_n \omega_j^{n-1}\frac{t^n}{n!}\right)$$
where the $B_n$ are the usual Bernoulli numbers. 
\end{general}

The classic Bernoulli polynomials are obtained with the choice $r = 1$, $\omega_1 = 1$, and the Bernoulli numbers are obtained for $z = 0$. These polynomials obey many relations which we sum up below and which can be easily obtained from the properties of the generating function.

\begin{general}{Proposition}
For $\omegabar \in \cc^{r},~ (\prod_{1 \leq j \leq r} \omega_j^{-1}) B_{r,n}(z, \omegabar)$ is a polynomial in $r+1$ variables, of degree $n$, which is symmetric in the $r$ variables of $\omegabar$.
If $\alpha \in \cc$, $\alpha \neq 0$, then 
\begin{align}
B_{r,n}(\alpha z, \alpha \omegabar) & = \alpha^{n-r} B_{r,n}(z, \omegabar) \nonumber \\
B_{r,n}(z + |\omegabar|, \omegabar) & = (-1)^n B_{r,n}(-z, \omegabar) \nonumber \\
B_{r,n}(z + \omega_j, \omegabar) & = B_{r,n}(z, \omegabar) + nB_{r-1,n-1}(z, \omegabar^{-}(j)) \nonumber \\
B_{r,n}(z + \omega_j, \omegabar) & = -B_{r,n}(z, \omegabar[j]) \nonumber \\
\partialdx{z}B_{r,n}(z, \omegabar) & = nB_{r,n-1}(z, \omegabar) \nonumber
\end{align}
\end{general}

The modular property for the $G_r$ functions involve these Bernoulli polynomials as proven by Narukawa in \pendingref.

\begin{generalbis}{Theorem}{[7 and 8 in \cite{Narukawa}]}
\label{Narukawa}
Let $r \geq 0$. Suppose $\omegabar \in (\cc - \rr)^{r+2}$ and $\omega_j/\omega_n \in \cc - \rr$ for all $j \neq n$. Then 
\begin{equation} \label{modGr}
\prod_{j = 0}^{r+1} G_r\left(\frac{z}{\omega_j}, \left(\frac{\omega_n}{\omega_j}\right)_{n \neq j}\right) = \exp\left(\frac{-2i\pi}{(r+2)!}B_{r+2,r+2}(z, \omegabar)\right)
\end{equation}
\end{generalbis}

\noindent The way Narukawa proves this identity uses multiple sine functions and their integral representations. We shall give a different proof of this theorem now using Lipschitz' formula and Eisenstein summation. 

\pending other proof



















==> geometric_setup/grfunctions/lattices.tex <==
\subsection{An analogue construction for $G_r$}

In this section we generalize the construction of section \pendingref for $G_r$ with $r \geq 0$.

\begin{general}{Definition}
Let $\abar$ be a family of $r+1$ independent primitive elements of $\zz^{r+2}$. There is a unique $s \in \zz$ and a unique primitive $\gamma \in \dual{\zz^{r+2}} = L$ such that $\forall c \in \zz^{r+2},~ \det(\abar, c) = s\gamma(c)$. Choose linear maps $\alpha_j \in L$ such that for all $0 \leq j \leq r$ :
$$\alpha_j(a_j) > 0~,~ \alpha_j(a_n) = 0, \forall n \neq j$$
We put 
$$G_{r, \abar}(w, x) = \prod_{\delta \in F/\zz\gamma} G_r\left(\frac{w+\delta(x)}{\gamma(x)}, \frac{1}{\gamma(x)}\alphabar(x) \right)$$
$$F = \{ \delta \in L, \forall 0 \leq j \leq r,~0 \leq \delta(a_j) < \alpha_j(a_j) \}$$
\end{general}

\noindent This is seen to be convergent for $\gamma(x) \neq 0,~\alpha_j(x)/\gamma(x) \not\in \rr$ for all $j$ and for suitable $w$ given by the convergence conditions for the regular $G_r$. We can easily check by direct computation that this definition does not depend on the choice for the $\alpha_j, 0 \leq j \leq r$. A choice that is interesting for us is once again defined by the comatrix or rather by the rescaled comatrix. Let $c$ be a vector such that $\gamma(c) = 1$. Then the elementary divisors of $(\abar, c)$ can be written as $[B_r, B_{r-1}, \dots, B_1, 1, 1]$ with $B_i | B{i+1}$ so that a possible choice for $\alphabar$ is given by :

$$\begin{pmatrix} \abar & c \end{pmatrix} \begin{pmatrix} \alphabar \\ B_r\gamma\end{pmatrix} = B_rI_{r+2}$$


To express the transformation properties of the function $G_{r, \abar}$ under the action of $\slnz{r+2}$ we need the following polynomials which generalise $P_{a,b,c}$:

\begin{general}{Definition}
Let $w \in \cc$ and $x \in \Lambda_{\cc}$. Let $a_0, \dots, a_r, a_{r+1}$ be $r+2$ primitive independent vectors in $\zz^{r+2}$. We put :
$$P_{r, \abar}(w, x) = \frac{-2}{(r+2)!} \sum_{\delta \in F(\alphabar)} B_{r+2,r+2}(w + \delta(x), \alphabar(x))$$ 
where $\alphabar$ is taken as above and
$$F(\alphabar) = \{\delta \in L, 0 \leq \delta(a_j) < \alpha_j(a_j), \forall 0 \leq j \leq r+1 \} $$ 
\end{general}

\noindent This definition will reveal to be independent of the choice of $\alphabar$ as we will show, and the $P_{r,\abar}$ are polynomials in $w$ of degree $r+2$ related to generalized Bernoulli polynomials. We can now generalize the result of section \pendingref.

\begin{general}{Theorem}
For all permutation $\sigma \in \goth{S}_{r+2}$
$$G_{r,\sigma(\abar)}(w,x) = G_{r,\abar}(w,x)^{\varepsilon(\sigma)}$$
Furthermore, we have the $r+2$-term relation
$$\prod_{j= 0}^{r+1} G_{r, ((a_n)_{n \neq j}}(w, x) = \exp(i\pi P_{r,\abar}(w,x))$$
The equivariance relations for $G_{r, \abar}$ and $P_{r, \abar}$ are written as follows with $g \in \slnz{r+2}$:
$$G_{r,g\abar}(w, gx) = G_{r,\abar}(w, x) $$
$$P_{r,g\abar}(w, gx) = P_{r,\abar}(w, x) $$
\end{general}

\begin{general}{Lemma}
For $g \in \slnz{r+2}$,
$$P_{r, g\abar}(w, gx) = P_{r,\abar}(w,x)$$
\end{general}
\begin{proof}
When considering $g\abar$, we replace $\alphabar$ by $\alphabar g^{-1}$ and $F(\alphabar)$ by $F(\alphabar)g^{-1}$. Therefore we can write :
$$P_{r, g\abar}(w, gx) = \frac{-2}{(r+2)!} \sum_{\delta \in F(\alphabar)g^{-1}} B_{r+2,r+2}(w + \delta(gx), \alphabar(x))$$
We put $\delta g^{-1} = \delta'$:
$$P_{r, g\abar}(w, gx) = \frac{-2}{(r+2)!} \sum_{\delta' \in F(\alphabar)} B_{r+2,r+2}(w + \delta(x), \alphabar(x))$$
$$P_{r, g\abar}(w, gx) = P_{r, \abar}(w, x)$$
\end{proof}

\begin{proof}
Switching two vectors in $\abar$ changes the sign of the determinant and therefore replaces $\gamma$ by $-\gamma$. Then, using the relation
$$G_r(-z, -\taubar) = \frac{1}{G_r(z, \taubar)}$$
for each term we get the result. The cyclic relation is a consequence of the modular property \refp{modGr} (see page \pageref{modGr}) for the regular $G_r$ function. Write the comatrix relation with primitive elements $\alpha_j$ and positive integers $s_j$ as :
$$\begin{pmatrix} a_0 & \dots & a_{r+1}\end{pmatrix} \begin{pmatrix} s_0 \alpha_0 \\ \dots \\ s_{r+1} \alpha_{r+1}\end{pmatrix} = sI_{r+3} $$
Write $F(\alphabar) = \{\delta \in L, 0 \leq \delta(a_j) < \alpha_j(a_j), \forall 0 \leq j \leq r+1\}$ so that we have the following formula for the $G_{r, ((a_k)_{k > j}, (a_k)_{k < j})}$:
$$G_{r, ((a_n)_{n > j}, (a_n)_{n < j})}(w, x) = \prod_{\delta \in F(\alphabar)} G_r\left(\frac{w + \delta(x)}{\alpha_j(x)}, \left(\frac{\alpha_n(x)}{\alpha_j(x)}\right)_{n \neq j} \right)$$
Using \refp{modGr} (page \pageref{modGr}) for each $\delta$ we get
$$\prod_{j= 0}^{r+1} G_{r, ((a_n)_{n > j}, (a_n)_{n < j})}(w, x) = \prod_{\delta \in F(\alphabar)} \exp\left(-\frac{2i\pi}{(r+2)!}B_{r+2, r+2}(w+\delta(x), \alphabar(x))\right)$$
We recover the polynomial $P_{r, \abar}(w,x)$ as :
$$P_{r, \abar}(w, x) = \frac{-2}{(r+2)!} \sum_{\delta \in F(\alphabar)} B_{r+2,r+2}(w + \delta(x), \alphabar(x))$$ 
So that 
$$\prod_{j= 0}^{r+1} G_{r, ((a_n)_{n > j}, (a_n)_{n < j})}(w, x) = \prod_{\delta \in F(\alphabar)} \exp\left(i\pi P_{r, \abar}(w, x)\right)$$
In particular, this proves that the definition of $P_{r, \abar}$ does not depend on the choice for $\alphabar$. For the equivariance, we write, with $\alpha_j$ replaced by $\alpha_j g^{-1}$ and $\gamma$ replaced by $\gamma g^{-1}$: 
$$G_{r, g\abar}(w, gx) = \prod_{\delta \in F(\alphabar g^{-1})/\zz\gamma g^{-1}} G_r\left(\frac{w + \delta(gx)}{\gamma(x)}, \frac{1}{\gamma(x)} \alphabar(x) \right) $$
because $\alpha(g^{-1}gx) = \alpha(x)$. Then, we have once again $F(\alphabar g^{-1}) = F(\alphabar)g^{-1}$ so that putting $\delta' = \delta g$ we have
$$G_{r, g\abar}(w, gx) = \prod_{\delta \in F(\alphabar)/\zz\gamma} G_r\left(\frac{w+\delta(x)}{\gamma(x)}, \frac{1}{\gamma(x)}\alphabar(x) \right) = G_{r, \abar}(w, x)$$
\end{proof}

\pending Zudilin remark


















==> geometric_setup/quadratic.tex <==
\subsection{The quadratic case}























































==> numerical/lowkappa3_old.tex <==
\stepcounter{example}
\subsubsection{Example \exc}
We now discuss a case where $q = 7$, $\kappa = 1$ and $\zfone \simeq \{-1, +1\}$. Consider $\zexc$ the complex root of the polynomial $x^4 - x^3 - x^2 - 5x + 1$ lying in the upper half-plane. Then $\kk_{\exc} = \qq(\zexc)$ has class number $1$. We choose $\goth{f} = \goth{P}_7$ the degree one prime above $7$ in $\kk_{\exc}$. We choose the fundamental units
$$\eps_1 = 2\zexc^3 - 5\zexc^2 + \zexc ,~\eps_2 = -\zexc^3 + \zexc^2 + 3\zexc$$
for $\opc{\goth{f}}$. We compute $\tlambda_1 = \tlambda_2 = 1$, $\ttt_1 = 13\cdot1069$, $\ttt_2 = 227257$ where $1069, 227257$ are prime numbers. We may choose $\goth{b} = (1)$ and $\goth{a}$ a degree one prime above $5$ in $\kk_{\exc}$. We search for target ideals and find $\goth{P}_{13}$ the degree one prime above $13$ and $\goth{P}'_{1069}$ a degree one prime above $1069$ in the first case. In the second case, we find $\goth{P}_{227257}$ a degree one prime above $227257$ in the second case. In Proposition \ref{propfinal} we may choose $m_1 = 3$, $m_2 = 1$ and $\goth{I} = \ok$ such that both ideals $3qN\goth{P}_{13}\goth{P}'_{1069}/\goth{a}$ and $qN\goth{P}_{227257}/\goth{a}$ are principal with admissible generators $h_1 = -336\zexc^3 + 189\zexc^2 - 21\zexc + 1323$ and $h_2 = 91\zexc^3 + 91\zexc^2 - 224\zexc - 413$. The corresponding levels will be $l_1 = 5\cdot7\cdot13\cdot1069$ and $l_2 = 5\cdot7\cdot227257$. Let us write the parameters

\begin{align*}
&\tau = \frac{5\eps_1\eps_2-1777937\eps_1+51}{\eps_1}, && \tau' = \frac{-29444256\eps_2\eps_1+276\eps_2-191}{\eps_1\eps_2} \\
&\sigma = \frac{-17935869\eps_1\eps_2+692\eps_1-197}{\eps_1 \eps_2}, && \sigma' = \frac{197\eps_2\eps_1+4832\eps_2+19040134}{1} \\
&\rho = \frac{-49\eps_1\eps_2-276\eps_1-2579783}{1}, && \rho' = \frac{216\eps_2\eps_1-3235133\eps_2-5}{\eps_2}
\end{align*}

\noindent Then 
$$ \prod_{k = 1, 6}\frac{G_2\left(\frac{3k}{7}, \frac{\tau}{486395}, \frac{\sigma}{486395}, \frac{\rho}{486395}\right)^{5}}{G_2\left(\frac{15k}{7}, \frac{\tau}{97279}, \frac{\sigma}{97279}, \frac{\rho}{97279}\right)} \times \frac{G_2\left(\frac{-k}{7}, \frac{\tau'}{7953995}, \frac{\sigma'}{7953995}, \frac{\rho'}{7953995}\right)^{-5}}{G_2\left(\frac{-5k}{7}, \frac{\tau'}{1590799}, \frac{\sigma'}{1590799}, \frac{\rho'}{1590799}\right)^{-1}}
$$
is close to the a number $\approx 46124.2850620... - i\cdot3503.2596737...$ whose $5$-th power is close to the root $\approx 196752223225284800050585.5328371... - i\cdot 78365336721542184758627.3801894...$ of the relative polynomial 
$(x^6+1) + (ay^3+by^2+cy +d)(x^5+x) +(a'y^3+b'y^2+c'y+d')(x^4+x^2) +(a''y^3+b''y^2+c''y +d'')x^3$ where
\begin{align*}
a &= -182042576709760837525764 \\
b &= 416567205193460328373593 \\
c &= 11453837546245488685752 \\
d &= 16195570033689796117050 \\
a' &= 38118142969638964328534610940657346948077979471 \\
b' &= 74233058267654907491296031652054558107892210823 \\
c' &= 34754348235503915169412485785829814479686421659 \\
d' &= 9111675109871182080469179191851629176480346002 \\
a'' &= -70345059350565384445770799625528928087524308811 \\
b'' &= 406696325982268482196474177889208303146072639191 \\
c'' &= 607519773193408407492767851761996343852214484427 \\
d'' &= 101932182631305576282017459590450601719066123283
\end{align*}
This relative polynomial defines $\kk_{\exc}^{+}(\goth{f})/\kk_{\exc}$. The computation time for $1000$ digits is 120 minutes.







